Not All Edges are Equally Robust: Evaluating the Robustness of Ranking-Based Federated Learning

Federated Ranking Learning (FRL) is a state-of-the-art FL framework that stands out for its communication efficiency and resilience to poisoning attacks. It diverges from the traditional FL framework in two ways: 1) it leverages discrete rankings instead of gradient updates, significantly reducing communication costs and limiting the potential space for malicious updates, and 2) it uses majority voting on the server side to establish the global ranking, ensuring that individual updates have minimal influence since each client contributes only a single vote. These features enhance the system's scalability and position FRL as a promising paradigm for FL training. However, our analysis reveals that FRL is not inherently robust, as certain edges are particularly vulnerable to poisoning attacks. Through a theoretical investigation, we prove the existence of these vulnerable edges and establish a lower bound and an upper bound for identifying them in each layer. Based on this finding, we introduce a novel local model poisoning attack against FRL, namely the Vulnerable Edge Manipulation (VEM) attack. The VEM attack focuses on identifying and perturbing the most vulnerable edges in each layer and leveraging an optimization-based approach to maximize the attack's impact. Through extensive experiments on benchmark datasets, we demonstrate that our attack achieves an overall 53.23% attack impact and is 3.7x more impactful than existing methods. Our findings highlight significant vulnerabilities in ranking-based FL systems and underline the urgency for the development of new robust FL frameworks.

==> sections/Acknowledgements.tex <==
% \section{Acknowledgements}
% We thank the anonymous reviewers and the shepherd
% for their valuable feedback.

==> sections/Ethical.tex <==
% \section*{Ethics Considerations and Compliance with the Open Science Policy}
% \noindent{\textbf{Ethics Considerations.}} In this study, our primary objective is to highlight the vulnerabilities in ranking-based FL systems, i.e., FRL, with the aim of encouraging the development of more robust and secure frameworks in the field. By identifying these weaknesses, we hope to contribute to enhancing security within the AI domain, ultimately leading to safer and more trustworthy AI systems.

% Our experiments were carefully designed and conducted within controlled environments to ensure that any risks to real-world systems or users were minimized. The methods and tools utilized in our research were based entirely on publicly available resources, ensuring transparency and reproducibility. Importantly, our study did not involve the use of personal data or human subjects, further mitigating ethical concerns.\\
% % We believe that by shedding light on these vulnerabilities, our work will inspire further research and development aimed at fortifying FL systems against potential threats, thereby advancing the overall security of AI technologies.

% \noindent{\textbf{Compliance with the Open Science Policy.}}
% In compliance with the open science policy, we are committed to making our research artifacts, including the source code, freely available online following the acceptance of this paper. By sharing these resources, we aim to foster transparency, reproducibility, and collaboration within the research community. Additionally, we are prepared to provide supplementary analysis results and data upon request.

==> sections/ab.tex <==
\section{Ablation Study}

==> sections/defense.tex <==


	
				








==> sections/frl.tex <==
\section{Federated Rank Learning}
\label{sec:frl}
\subsection{Formulation of FRL}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figures/FRL.pdf}
    \caption{FRL.}
    \label{fig:FRL}
\end{figure*}

The objective of FRL is to find a global ranking $R_g$, such that the resulting subnetwork $\theta^w \odot m$ minimizes the average loss of all clients:
\begin{equation}
\begin{alignedat}{2}
& \min_{R_g} F(\theta^w, R_g) = \min_{R_g} \sum_{u=1}^U{\lambda_i L_i(\theta^w \odot m)} \quad \\
&\text{s.t. } \\
& m[R_g < k] = 0 \text{ and } m[R_g \geq k] = 1,
\end{alignedat}
\end{equation}
where $U$ is the total number of FRL clients, $\theta^w$ is the randomly initialized global weight, $L_i$ is the loss function for the $i^{th}$ client, $\lambda_i$ is the importance, e.g., weight, of the $i^{th}$ client. $m$ is the final binary mask used to select the edges for \textit{subnetowork}. It consists of three steps: \\
% Specifically, consider an edge $E_{uv}$ that connects two neurons $u$ and $v$, $W_{uv}$ be the weight of $E_{uv}$, and $s_{uv}$ be the score assigned to the edge $E_{uv}$.
\textbf{Server Initialization:}
As shown in Figure \ref{fig:FRL} (a), in the first round, the FRL server chooses a random seed to generate initial random weights $\theta^w$ and scores $\theta^s$ for the global \textit{supernetwork}; 
Then, it sorts the scores $\theta^s$ in ascending order to get the corresponding ranking $R_g$.
% i.e., $R1g = ARGSORT(\theta^s)$. We define rankings of a vector as the indices of elements of vector when the vector is sorted from low to high, which is computed using ARGSORT function.
% Next, the FRL server shares seed with FRL clients, who can then locally reconstruct the initial weights $\theta^w$ and scores $\theta^s$.
Since $R$ stores two-dimensional information, e.g., edge number and corresponding ranking, we expand $R$ to the two-dimensional matrix to have a better understanding of $R$ and reduce some undifferentiable operation proposed in FRL \cite{mozaffari2023every}. Therefore, we have the following definition. \\
\textbf{\textit{Definition 1}} (Permutation Matrix): An $n \times n$ binary matrix $P \triangleq (P_{i,j})_{i,j} \in [1,n] \in \{0,1\}^{n \times n}$ is called a \textit{permutation matrix} if and only if 
\begin{equation}
    \forall i,j \in [0,n], \sum_{i' \in [0,n]} P_{i',j}=1,\sum_{j' \in [0,n]} P_{i,j'}=1.
\end{equation}\\
% The set of $n \times n$ permutation matrices is denoted by $X_n$. The cardinality of $X_n$ is $n!$.
% For example, if $n=3$, then $X_n$ is given by
% \begin{align*}
% X_n &= \left\{ \begin{bmatrix} 1 & 0 & 0 \\ 0 & 1 & 0 \\ 0 & 0 & 1 \end{bmatrix}, \,
% \begin{bmatrix} 0 & 1 & 0 \\ 1 & 0 & 0 \\ 0 & 0 & 1 \end{bmatrix}, \,
% \begin{bmatrix} 0 & 0 & 1 \\ 0 & 1 & 0 \\ 1 & 0 & 0 \end{bmatrix}, \right. \\
% &\quad \left. \begin{bmatrix} 1 & 0 & 0 \\ 0 & 0 & 1 \\ 0 & 1 & 0 \end{bmatrix}, \,
% \begin{bmatrix} 0 & 0 & 1 \\ 1 & 0 & 0 \\ 0 & 1 & 0 \end{bmatrix}, \,
% \begin{bmatrix} 0 & 1 & 0 \\ 0 & 0 & 1 \\ 1 & 0 & 0 \end{bmatrix} \right\}
% \end{align*}
% The permutation function $\Pi: X \rightarrow X$ is a bijection that maps the element of $X$ to itself.\\
Let $E=[e_0,e_1,...e_{N-1}]$ denote the edges in each layer. $P_u$ denotes a $N \times N$ \textit{permutation matrix} computed from user $u \in U$ s.t., $P_u=R_u^\top \cdot E$, where $N$ is the number of edges in each layer.
For instance, as shown in Fig. \ref{fig:FRL}, the initial global ranking is $R_g=[0,1,4,3,2,5]$, meaning that edge $e_0$ is the least important edge (in the first position) and $e_5$ is the most important edge (in the last position). In the generate $P_g$, each column indicates each edge number ($e_1,e_2,\dots,e_5$), while each row indicates the position in the ranking. $P_{1,1}=1$ meaning that edge $e_0$ is in the first position of $R_g$, $P_{6,6}=1$ meaning that $e_5$ is in the sixth position.
Note that the $P_u$ generated from $R_u$ have the exact same meaning but can be calculated in a differentiable manner. Therefore, we use $P_u$ to perform the following aggregation process.\\
\textbf{Client Training:} On the client side, the client uses the edge-popup (EP) algorithm \cite{ramanujan2020s} to update the score of each edge.
% therefore, to get the corresponding ranking $R_i$.
% The edge-popup algorithm removes edge $e$ from the supermask if its score is not within the top $k$ highest scores.
In each iteration of client training, clients update the scores of all edges such that if having an edge $e$ in the subnetwork reduces loss (e.g., cross-entropy loss) over training data, the score of $e$ increases.
Detailed steps can be seen in Appendix \ref{alg:ep}.
Then, clients send the updated ranking matrix $P_u$ to the server for aggregation. \\
\textbf{Server Aggregation:} The server receives all the local rankings of the selected $u$ clients, i.e., $P_u \{u \in U\}$, and uses majority voting (MV) to get the aggregated ranking.  
Specifically, the server first calculates dimension-wise summarization of the received $P_u$, e.g., $S = \sum_{u=0}^{U-1} P_u$ to get the aggregated ranking matrix $S$.
% Note that all FRL operations that involve sorting, reordering, and voting are performed in a layer-wise manner. For instance, the server computes global rankings $R_t^g$ in round $t$ for each layer separately, and consequently, the clients selected in round $t$ reorder their local randomly generated scores $\theta^s$ for each layer separately.
Since each column in $S$ indicates the edge and each row indicates the position in $R$.
Then, we can get the relative important weight for each edge: 
\begin{equation}
\begin{alignedat}{2}
\label{eq:weight}
w_j&=\sum_{i=0}^{N-1}\alpha_i S_{i,j}\\
&=\textbf{A} \cdot S_j,
\end{alignedat}
\end{equation}
where $\textbf{A}$ is a row vector indicating the scaling factor, following the FRL \cite{mozaffari2023every}, we use the value of $i$ as the weight for position $i$, e.g., $\alpha_i=i$, therefore $\textbf{A}=[1,2, \dots, N]$.\\
Lastly, the server sorts the $w$ in ascending order, and top $k$ edges are selected for the \textit{subnetwork}.
Therefore, the MV function can be formulated as follows:
\begin{equation}
\begin{alignedat}{3}
\label{eq:wmv}
 R_g&=sort(f(R_{u \in U})) \\
    &=sort(g(\sum_{u=0}^{U} (P))) \\
    &=sort (\textbf{A} \cdot S) \\
    &=sort(\sum_{i=1}^{N} \alpha_{i} S_{i,0},\sum_{i=1}^{N} \alpha_{i} S_{i,1},...,\sum_{i=1}^{N} \alpha_{i} S_{i,N-1}),
\end{alignedat}
\end{equation}
% \begin{equation}
% \begin{alignedat}{3}
% \label{eq:wmv}
%  R_g&=\mathbb{M}(R_{u \in U}) \\
%     &=sort (f(R_{u \in U})) \\
%     &=sort (f(P_{u \in U} \cdot E ^\top)^\top) \\
%     % &=\mathbb{M}((P_{u \in U} \cdot E ^\top)^\top) \\
%     &=sort(\sum_{i=0}^{N-1} \alpha_{i} S_{i,0},\sum_{i=0}^{N-1} \alpha_{i} S_{i,1},...,\sum_{i=0}^{N-1} \alpha_{i} S_{i,n-1}),
% \end{alignedat}
% \end{equation}
where $f$ denotes the MV function and $g$ is the function to get the important weight of each edge.
% where $\alpha_{i}$ is the $i$th weight for the edge $j \in N$. We follow FRL to use the value of $i$ as the weight for $\alpha_{i}$ (e.g., $\alpha_{i}=i$).
% For simplicity, 
% we use $w_j=\sum_{i=0}^{N-1} \alpha_i S_{i,j}$ represents the relative importance weight of each edge $j$.
For simplicity, we denote $\textbf{w}=\{w_0,w_1,\dots,w_{(N-1)}\}$ as the important weight for each edge. 
% \subsection{Challenges of poisoning of FRL}
% Below are three reasons why FRL is hard to poison.\\
% \textbf{Less choice for malicious update:} 
% % FRL limits the choices of malicious clients update by enforcing a discrete space of updates (a permutation of integers $\in [1, N])$. 
% As shown in Figure \ref{fig:challenge}, most of the existing Byzantine robust FL algorithms use a continuous space of updates. They usually have a safe space where any update within this range will be accepted by the server for aggregation. In this frame, the adversary can generate malicious updates such that its maximum distance from any other gradient is upper
% bounded by the maximum distance between any two benign gradients \cite{jagielski2018manipulating}. This results in an infinite number of potential malicious updates.
% In contrast, in FRL, the clients send their updates in the form of edge rankings, which are permutations of integers within the range $[1, N]$ where $N$ is the number of edges in each layer; 
% This constraint significantly reduces the space for malicious updates from infinity to $N!$, thereby substantially mitigating the severity of potential attacks. \\
% % The discrete constraint also makes it harder for SGD-based optimizers to search for the optimal attack. 
% \textbf{Scale up the difference:} In traditional FL, adding a small perturbation on the beign gradient can have a significant impact on the global model

% \textbf{Don't involve gradient calculation:} Existing most effective poisoning attacks typically involve gradient manipulation to hinder the model's convergence or cause it to converge to a sub-optimal solution  \cite{jagielski2018manipulating,fang2020local}. However, FRL does not involve any gradients update as it uses randomly initialized model weights. Consequently, traditional model poisoning attacks cannot be directly applied to FRL. Conversely, data poisoning attacks \cite{munoz2017towards} are generally less effective than model poisoning attacks. 

==> sections/methods-old.tex <==
\section{Methods}
\subsection{Threat Model of model poisoning attacks}
To deal with the above challenges, we proposed our attack.\\
Here, we discuss the threat models of our poisoning attacks on FRL.\\
\textbf{Adversary’s Objective.} The adversary aims to launch an untargeted poisoning attack by generating malicious ranking $R'_m$ such that when the malicious clients update $R'_m$ with the central server, the accuracy of the resulting global \textit{subnetwork} reduces.\\
\textbf{Adversary’s Capabilities.} We assume that the adversary controls up to $m$ out of $U$ total clients, called malicious clients. We follow the previous setting \cite{fang2020local,shejwalkar2021manipulating}, assuming that the number of malicious clients is less than the number of benign clients, i.e., $(m/U) < 0.5$.
For adversary’s knowledge, we consider two cases: \textit{update-aware} and \textit{update-agnostic}. In \textit{update-aware} setting, we assume the attacker has access to $m$ benign update (different from the previous assumption, \cite{fang2020local,shejwalkar2021manipulating} where the adversary needs to have access to all benign updates). Although \textit{update-aware} adversary has limited practical significance, this scenario has been commonly used in prior works \cite{fang2020local,shejwalkar2021manipulating,baruch2019little} to assess the severity of the poisoning attack. 
In \textit{update-agnostic} setting, the adversary does not have any information of benign updates. 
\subsection{Optimization function:}
\subsubsection{Optimization Function}
Our optimization problem aims to maximize the damage to the global model in each iteration. Therefore, we aim to generate $m$ malicious update $R'_m$
such that the global model's importance weight of each edge $e$ is far from the original \textit{benign} model.
Therefore, the objective of the full-knowledge adversary is given by:
\begin{equation}
\label{eq:objective}
\begin{alignedat}{2}
& \arg\max_{R'_1,R'_2,\dots,R'_m} \left\| \textbf{w}- \textbf{w}' \right\| \\
& \text{s.t.} \\
&\textbf{w}=f(R_1, \dots R_m, R_{m+1}, \dots,R_U) \\
&\textbf{w}'=f(R'_1, \dots R'_m, R_{m+1}, \dots,R_U)
\end{alignedat}
\end{equation}
where $\textbf{w}$ is the importance vector before the attack and $\textbf{w}'$ importance vector after the attack. $|| \cdot ||$ denote the Euclidean norm given by $|| x || \triangleq (x^T x)^{1/2}$.

The aggregated ranking matrix before the attack is $S = S^b+S^m$ and the aggregated ranking matrix after the attack is $S'=S^b+S^{m'}$, where $S^b$ is the aggregation of $U-m$ benign updates, $S^m$ is the aggregation of $m$ benign updates and $S^{m'}$ is the aggregation of $m$ malicious updates. 
Additionally, we use $R'= R \cdot P$ to denote the malicious update, where $P$ is the permutation matrix.
Therefore, Eq \ref{eq:objective} can be further calculated as:
\begin{equation}
\label{eq:object-3}
\begin{alignedat}{5}
& \arg\max_{P_1,P_2,\dots,P_m} \left\| \textbf{w}- \textbf{w}' \right\| \\
& \text{s.t.} \\
&\textbf{w}=f(R_1, \dots R_m) \\
&\textbf{w}'=f(R_1 \cdot P_1, \dots R_m \cdot P_m)
\end{alignedat}
\end{equation}



% Thus, our optimization function becomes Eq.\ref{eq:objective-two}
\subsubsection{Searching Range}
The critical challenge of solving the optimization problem is that the search space of $P_m$ is large, e.g., $mN!$. To address the challenge, 
% we make two approximations. Our approximations represent suboptimal solutions to the optimization problem. However, as we will demonstrate in our experiments, our attacks already substantially increase the error rate of the learned model.
we first define a search range $j \in \{t_1,t_2\}$, where we only make modifications of $P_m$ in this range. This relaxation has several advantages: 
firstly, we will demonstrate in section \ref{} that this relation will achieve equivalent or even better effects compared to making modifications on every edge. 
Secondly, since we only make modifications on a small amount of edges, it has a far smaller chance of being detected, as demonstrated in Section \ref{}.
Lastly, it also largely reduces the time and memory usage for the optimization process, which will be further discussed in Section \ref{}.
% Additionally, we further.
We further illustrate how to find the threshold $t_1$ and $t_2$.\\
\textbf{Theorem 1.} 
Let $k$ be the edge of the smallest weight $w_k$ that is selected by the \textit{subnetwork}. Assume $v$ is an edge not selected by the model before the attack, such that $ w_v < w_k $. To ensure a successful attack, $w_k$ needs to satisfy the following condition:
\begin{equation}
\label{eq:bound}
w_k-w_v<m (N-1),
\end{equation}
% \textbf{Theorem 2.}
Similarly, assume $y$ is an edge that is selected by the model before the attack s.t., $w_k \leq w_y$. 
To ensure a successful attack, $w_y$ needs to satisfy the following condition:
\begin{equation}
\label{eq:bound_2}
w_y-w_k<m (N-1).
\end{equation}
Thus we define our search region as $j \in [t_1:t_2]$, where 
% $\sum_{i=0}^{N-1} \alpha_i (S_{i,k}-S_{i,t_1})=\sum_{i=0}^{N-1} \alpha_i (S_{i,t_2}-S_{i,k})= m (N-1)$.
 $\textbf{A} \cdot (S_{k}-S_{t_1})=\textbf{A} \cdot (S_{t_2}-S_{k})= m (N-1)$.
Since we assume the adversary only knows $m$ benign users update, we use the aggregation of $m$ benign clients to get an estimated value of all $U$ users to calculate the threshold:
\begin{equation}
\label{eq:estimiated_threshold}
S=U/m*S^m.
\end{equation}
\\



\subsection{Solve Optimization Function}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figures/attack.pdf}
    \caption{Attack.}
    \label{fig:attack}
\end{figure*}

\begin{algorithm}
\caption{Attack process.}
\label{alg:attack}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}



\Require $m$ benign rankings $R_s$, $u$ number of clients selected for current round, $m$ number of malicious clients, $k$ subnetwork sparsity, number of epoch $E$, $L$ iterations for Gumbel-Sinkhorn training, $\tau$ tempaure factor for Gumbel-Sinkhorn,
learning rate $\eta$.

\Ensure $R'_1,R'_2,\dots,R'_m$
\State \textbf{Initialization:}
\State $t_1, t_2 \gets \Call{get\_threshold}{R_s, u, m, k}$
\State $X \gets \text{m continues matrix of size }  (t_2 - t_1) \times (t_2 - t_1)$
\State \textbf{Optimization:}
\For{$e \in E$}
    \State $P \gets \Call{Gumbel\_Sinkhorn}{X, L, \tau}$
    \State $X=X- \eta \nabla \ell(R_s;X)$
\EndFor
\State $P \gets \Call{Hungarian\_algorithm}{P}$
\State $R_s'=R_s \cdot P$
\For{$i \in m$}
    \State $R'_i=R'_s[i]$
\EndFor
\Function{Gumbel\_Sinkhorn}{$X, L,\tau$}
    \State \textbf{Initialization:} 
    \State $S_0(X) \gets \exp(X)$
    
    \State \textbf{Normalization:}
    \For{$l = 1, 2, \ldots L$}
        \State $S^l(X) \leftarrow T_c(T_r(S^{l-1}(X)))$
    \EndFor
    \State $P \leftarrow S^L(X)$
    \State \textbf{Approximation:}
    \State $h(P) \leftarrow - \sum_{i,j} P_{i,j} \log (P_{i,j})$
    \State $S(X/\tau) \leftarrow \arg \max_{P \in B_N} \langle P, X \rangle_F + \tau h(P)$
    \State \Return $S(X/\tau)$

    
    % \State \textbf{Discrete Matching:}
    % \State $M(X) \leftarrow \lim_{\tau \to 0^+} S(X/\tau)$
\EndFunction

\end{algorithmic}
\end{algorithm}

In previous sections, we formulated our optimization function such that the final objective is to find the $m$ permutation matrix $P_m$ that can maximize the weight difference.\\
\textbf{Softmax for Permutations:}
Since permutation matrices are discrete and cannot be directly optimized, a practical approach is to transform a discrete matrix into a continuous one. Specifically, given a matrix $X$ from a continuous distribution, we aim to convert it into a permutation matrix by focusing on the largest values in $X$. By using this method, we can employ the Adam optimization algorithm \cite{kingma2014adam} to optimize $X$, which will concurrently update the permutation matrix $P$ that we need to obtain.
Therefore, we have the following definition:\\
\textbf{\textit{Definition 2}} (Matching Operation): Given a matrix $X$ drawn from a continuous distribution, we aim to map $X$ to a permutation matrix based on its values. Specifically, we want to select the biggest value in each row and column to set as 1 and others as 0, at the same time making sure the sum of each row and each column is 1. 
To achieve this, we define the following matching operator $M(X)$ for our discrete optimization:
\begin{equation}
\label{eq:matching}
M(X) = \arg \max_{P \in P_N} \langle P, X \rangle_F,
\end{equation}
where $P_N$ denoting the set of permutation matrices and $\langle P, X \rangle_F = \text{trace}(A^\top B)$ is the (Frobenius) inner product of matrices.

Since the Matching Operation is still not differentiable, we seek a continuous method that can approximate this discrete operation. To achieve this, we employ the Gumbel-Sinkhorn approach \cite{mena2018learning}. 
The Gumbel-Sinkhorn method combines ideas from the Gumbel-Softmax trick \cite{jang2016categorical} and the Sinkhorn algorithm \cite{adams2011ranking} to provide a way to sample from the set of permutation matrices in a differentiable manner. 
Based on the Gumbel-Sinkhorn algorithm,
we first use the Sinkhorn operator \cite{adams2011ranking} to normalize the rows and columns to get a doubly stochastic matrix:
\begin{equation}
\label{eq:Sinkhorn}
\begin{alignedat}{3}
S_0(X)& = \exp(X), \\
S_l(X)& = T_c(T_r(S_{l-1}(X))), \\
S(X)& = \lim_{l \to \infty} S_l(X),
\end{alignedat}
\end{equation}
where $T_r(X) = X \oslash (X 1_N 1_N^\top)$
and $T_c(X) = X \oslash (1_N 1_N^\top X)$ as the row and column-wise normalization operators of a matrix,
 \( 1_N \) is a column vector of ones of length \( N \), \( 1_N^\top \) is its transpose (a row vector of ones), and \( \oslash \) denotes element-wise division.\\
Then, we can use the following continuous method to approach Eq. \ref{eq:matching}:
\begin{equation}
S(X/\tau) = \arg \max_{P \in B_N} \langle P, X \rangle_F + \tau h(P),
\end{equation}
where $B_N$ is the set of doubly-stochastic matrices, $\tau$ is a positive temperature parameter, and $h(P) = - \sum_{i,j} P_{i,j} \log (P_{i,j}))$ is the entropy of matrix $P$.
And \(M(X)\) can be obtained as the limit of \(S(X/\tau)\), meaning that one can approximate \(M(X) \approx S(X/\tau)\) with a small \(\tau\):
\begin{equation}
\label{eq:lim}
M(X) = \lim_{\tau \to 0^+} S(X/\tau).
\end{equation}
Since Eq. \ref{eq:lim} cannot be realized in practice, as it involves a limit on the Sinkhorn iterations $L$ and the temperature $\tau$. Therefore, after the optimization process, we use the Hungarian algorithm \cite{mills2007dynamic} to get the exact permutation matrix from the doubly stochastic matrix. Specifically, we use the doubly-stochastic matrix obtained from Eq. \ref{eq:lim} as the cost matrix and use the Hungarian algorithm to find the optimal assignment that maximizes the total cost.
\subsection{Attack process}
Algorithm \ref{alg:attack} and Figure \ref{fig:attack} demonstrate the detailed process of our attack. In this initialization stage, the adversary gets the $m$ benign rankings and stores them in a $(m \times N)$ tensor, denoted as $R_s$.
Then, it uses benign rankings to calculate the threshold of the search range (line 2). Then, it generates $m$ continued matrix of the size of $(t_2-t_1) \times (t_2 -t_1)$, denoted as $X$.
During the optimization stage, the adversary uses the Gumbel-Sinkhorn algorithm to iteratively optimize $X$ while concurrently updating the value of $P$ (lines 5 - 8). Then, it utilizes the Hungarian algorithm to convert $P$ to the exact permutation matrix (line 9). Lastly, the adversary performs the permutation on benign rankings using the optimized permutation matrices to get the malicious rankings $R_s'$ (line 10) and assign $R'_s[i]$ to each malicious user (lines 11 -13).
% \subsection{Complexity analysis}

==> sections/motivation.tex <==
\subsection{Threat Model of Model Poisoning Attacks}
% To deal with the above challenges, we proposed our attack.\\
%Here, we discuss the threat models of our poisoning attacks on FRL.\\

\noindent\textbf{Adversary’s Objective.} Since training an FL model is time-consuming and computationally intensive, injecting malicious clients into the training process to destroy the global model can pose a severe threat to FL \cite{shejwalkar2021manipulating}. Therefore, in this paper, we consider the untargeted local model poisoning attack, such that when the adversary shares the malicious update with the central server, the accuracy of the resulting global model reduces as much as possible.\\
\textbf{Adversary’s Capabilities.} We assume that the adversary controls up to $m$ out of $U$ clients for each iteration, called malicious clients. Each malicious client has its own clean dataset.
We follow the previous setting \cite{fang2020local,shejwalkar2021manipulating} and assume 
%that 20\% malicious client for each iteration, i.e., 
$m/U = 0.2$. \\
\textbf{Adversary’s knowledge.} We consider the \textit{update-agnostic} setting, where the adversary does not have any information of $U-m$ benign updates. 
%However, they have a set of clean datasets used to generate malicious updates.
However, the adversary will make use of the clean datasets from controlled clients to generate malicious updates.




\subsection{Motivation}
\label{sec:intuition}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/challenage.pdf}
    \caption{Motivating Example of Poisoning FRL. Top shows the `reverse rank' attack where all edge rankings are reversed; Middle shows `traditional poisoning attacks' that separate rankings into safe and unsafe spaces and reverse each separately; Bottom shows our attack, which targets and manipulates specific edges. Only our attack leads to changes in the global \textit{subnetwork}.}
    \label{fig:challenges}
\end{figure}
We begin by highlighting the key observations regarding the limitations of existing poisoning attacks on FRL, which motivates the development of our VEM.

To launch model poisoning attacks on FRL, the straw-man approach is to replace high-ranked edges with low-ranked ones in the malicious update, thereby negatively impacting the global model. In FRL \cite{mozaffari2023every}, the adversary computes the rankings based on  
its benign data and uses majority voting to simulate the aggregated ranking. Each malicious client then submits the reverse of this simulated global ranking to the FRL server for aggregation (we refer to it as a reverse-rank attack hereinafter). This attack is considered the `worst-case' untargeted poisoning attack on FRL in~\cite{mozaffari2023every}. However, this seems the strongest approach is ineffective for poisoning FRL. 
As shown in Fig. \ref{fig:challenges} (top), the first two rows represent benign updates (selecting edges [1,~6,~2]), while the third row represents malicious updates. Even though the malicious user reverses the ranking of every edge, it still results in the selection of edges [1,~6,~2] for the \textit{subnetwork} after majority voting. 
Furthermore, we examined other traditional poisoning attacks. The basic idea of traditional poisoning attacks is to make the malicious update relatively far from benign updates but still within a safe space to avoid detection. To implement this idea into FRL, we divided the ranking into two parts: safe space (top k\%) and unsafe space (others), and revised the ranking in these two parts separately. As shown in Fig. \ref{fig:challenges} (middle), 
after majority voting, the global model still selects edges [1,~6,~2] for the \textit{subnetwork}.

The failure of the above two examples lies in the fact that the ranking-based update imposes an upper bound on the adversary's potential damage, thereby minimizing their influence on the global model selection. Consequently, it becomes difficult for the minority to alter the voting outcomes against the majority.

However, we observe that FRL is not inherently robust, and there are specific edges that are particularly vulnerable to poisoning attacks. 
To verify this argument, we record the \textit{reputation} difference between each edge and the selection boundary $\gamma$, which is calculated as $\Delta_j = |w_j - \gamma|$, where $w_j$ is the \textit{aggregated reputation} for edge $e_j$ (for $j \in n$). 
This metric indicates the minimal modification needed for edge $e_j$ to cross the selection boundary, thereby reflecting its vulnerability. A lower value of $\Delta_j$ signifies a higher vulnerability.
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/difference_new2.pdf}
    \caption{\textit{Reputation} difference between each edge and the selection boundary. }
    \label{fig:difference}
\end{figure}
As illustrated in Fig. \ref{fig:difference}, there is a significant variation in $\Delta_j$ (for $j \in n$), ranging from 0 to 5616 for the MNIST dataset and from 0 to 17208 for the CIFAR10 dataset. Additionally, we use the red dash line to indicate the max adversary damage (e.g., 20\% malicious rate), the edges to the left of it are considered vulnerable edges. 
% Based on these observations, we raise two intriguing questions: 1) Is FRL inherently robust? In other words, with a limited number of malicious users, is it truly impossible to alter the voting results?
% 2)  If not, are there specific edges that are more vulnerable to poisoning attacks? If such edges exist, how can we identify those edges to launch a successful attack?

% They ignore the fact that different edges have different vulnerabilities to be altered across the selection boundary.  
% As shown in Fig. \ref{fig:difference}, 

% The failure of the above two attacks 
% lies in the fact that most benign clients agree on top-ranking edges; therefore, it is hard to alter the ranking of those highly agreed edges.
% However, it becomes vulnerable when malicious modifications are applied to edges near the selection boundary.  
% The answer to the first question is negative.
 
Based on the above observation, we update malicious ranking by manipulating only the vulnerable edges. As a result, the global model selects edges [5,~2,~6] for the \textit{subnetwork}, leading to a potential accuracy drop, as shown in Fig. \ref{fig:challenges} (bottom).
% This demonstrates that some edges are indeed vulnerable to poisoning attacks. 
% In other words, different edges exhibit varying degrees of vulnerability.
% Additionally, we also conducted experiments on Section \ref{sec:not_equal} to show a detailed demonstration of this observation.

% Based on this intuition, we give the factor to launch a successful attack in FRL: only manipulate the edges that are vulnerable to being altered. Therefore, for our attack, we first define a range where the edges inside this range can be considered vulnerable to attack. Then, we permute these vulnerable edges to get the optimal attack effect.
% Based on this intuition, we give the key factor to launch a successful attack in FRL: direct manipulation on the edges that are near the selection boundary. Therefore, for our attack, we first define a range where the edges inside this range can be considered vulnerable to attack. Then, we permute the ranking within this range to get the optimal attack effect.

% \subsection{Not all Edges are Equal}
% \label{sec:not_equal}
% In this section, we empirically address the questions raised in Section \ref{sec:intuition} and verify that different edges have different vulnerabilities for poisoning attacks.

% We consider a cross-device FL scenario where 1000 benign clients collaborate to train a global model using the FRL aggregation rule. In each training round, the server randomly selects 25 clients to participate in the \textit{subnetwork} selection. 
% Since this selection is based on the global ranking $R_g$, which is determined by the \textit{aggregated reputation} $W$. We utilize $W$ to evaluate the vulnerability of each edge. Specifically, 
% during each round, we record the \textit{reputation} difference between each edge and the selection boundary $\gamma$, which is calculated as $\Delta_j = |w_j - \gamma|$, where $w_j$ is the \textit{aggregated reputation} for edge $e_j$ (for $j \in n$). This metric implies the minimal modification needed for edge $e_j$ to cross the selection boundary. A lower value of $\Delta_j$ signifies a higher vulnerability.
% Since the \textit{subnetwork} selection is based on the global ranking $R_g$, which is determined by the \textit{aggregated reputation} $W$, we use the \textit{reputation} difference between each edge and the selection boundary to quantify the vulnerability for each edge.
% Specifically, we use
% $\Delta_j=|w_j-\gamma|$ to denote the \textit{reputation} difference between each edge $e_j$ and the selection boundary $\gamma$, where $w_j$ is the aggregated reputation for edge $e_j$. This measure also implies the minimal modification needed for edge $e_j$ to `cross the selection boundary'.
% An edge \(e_j\) is considered to have `crossed the selection boundary' if it satisfies
% \begin{equation}
%     e_j \in \mathbb{E}^{\text{in}} \text{ and } e_j \notin \mathbb{\widetilde{E}}^{\text{in}},
% \end{equation}
% or
% \begin{equation}
%    e_j \notin \mathbb{E}^{\text{in}} \text{ and } e_j \in \mathbb{\widetilde{E}}^{\text{in}},
% \end{equation}
% where $\mathbb{E}^{\text{in}}$ denote the top k\% edges selected for the \textit{subnetwork} before the attack and $\mathbb{\widetilde{E}}^{\text{in}}$ denote the top k\% edges after the attack. Then we use $\Delta_j=|w_j-\gamma|$ to denote the minimal modification needed for edge $e_j$ to `cross the selection boundary', where $w_j$ indicate the \textit{aggregated reputation} of edge $e_j$ and $\gamma$ indicate the selection boundary.
% Intuitively, if an edge is easier to alter across the selection boundary, we say that edge is more vulnerable to a poisoning attack. Therefore, to quantify this vulnerability, we measure the minimal effort required to make an edge cross the selection boundary. Since the subnetwork selection is determined by the ranking global $R_g$ and $R_g$ is determined by aggregated reputation. Therefore, we measure the  $\Delta_j=|w_j-\gamma|$ to denote the minimal modification needed for edge $e_j$ to `cross the selection boundary', where $w_j$ indicate the \textit{aggregated reputation} of edge $e_j$ and $\gamma$ is the selection boundary.
% We begin with the following definition.\\
% \textbf{Definition 1.}
% Let $\mathbb{E}^{\text{in}}$ denote the top k\% edges selected for the \textit{subnetwork} before the attack and $\mathbb{\widetilde{E}}^{\text{in}}$ denote the top k\% edges after the attack. 
% An edge \(e_j\) is said to `cross the selection boundary' if it satisfies
% \begin{equation}
%     e_j \in \mathbb{E}^{\text{in}} \text{ and } e_j \notin \mathbb{\widetilde{E}}^{\text{in}},
% \end{equation}
% or
% \begin{equation}
%    e_j \notin \mathbb{E}^{\text{in}} \text{ and } e_j \in \mathbb{\widetilde{E}}^{\text{in}}.
% \end{equation}
% And we use $\Delta_j=|w_j-\gamma|$ to denote the minimal modification needed for edge $e_j$ to `cross the selection boundary', where $w_j$ indicate the \textit{aggregated reputation} of edge $e_j$ and $\gamma$ indicate the selection boundary.
% then examine a scenario in which 25 benign clients collaboratively train an FRL model. 
% To quantify this vulnerability, we measure the minimal effort required to make an edge cross the selection boundary. We begin with the following definition.\\
% \textbf{Definition 1.}
% Let $\mathbb{E}^{\text{in}}$ denote the top k\% edges selected for the \textit{subnetwork} before the attack and $\mathbb{\widetilde{E}}^{\text{in}}$ denote the top k\% edges after the attack. 
% An edge \(e_j\) is said to `cross the selection boundary' if it satisfies
% \begin{equation}
%     e_j \in \mathbb{E}^{\text{in}} \text{ and } e_j \notin \mathbb{\widetilde{E}}^{\text{in}},
% \end{equation}
% or
% \begin{equation}
%    e_j \notin \mathbb{E}^{\text{in}} \text{ and } e_j \in \mathbb{\widetilde{E}}^{\text{in}}.
% \end{equation}
% And we use $\Delta_j=|w_j-\gamma|$ to denote the minimal modification needed for edge $e_j$ to `cross the selection boundary', where $w_j$ indicate the \textit{aggregated reputation} of edge $e_j$ and $\gamma$ indicate the selection boundary.
% !!!!!!!!!!!!!!!
% We then examine a scenario in which 25 benign clients collaboratively train an FRL model. During the training, we track the $\Delta_j$ for each edge $e_j$.
% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/difference_new2.pdf}
%     \caption{\textit{Reputation} difference between each edge and the selection boundary. }
%     \label{fig:difference}
% \end{figure}
% As illustrated in Fig. \ref{fig:difference}, there is a significant variation in $\Delta_j$, ranging from 0 to 5616 for the MNIST dataset and from 0 to 17208 for the CIFAR10 dataset. 
% Furthermore, we consider inserting $m$ malicious user to the FL system to affect the global ranking. Since \textit{reputation} ranges from 1 to $n$, the max \textit{reputation} change the adversary can cause for an edge is $nm$. 
% we use the red dashed line to represent the maximum \textit{reputation} change that the adversary can achieve ($nm$). Consequently, the edges to the left of the dashed line are vulnerable to attacks.


